Speech-to-Text Adapter and Speech-to-Entity Retriever Augmented LLMs for Speech Understanding

Large Language Models (LLMs) have been applied in the speech domain, often incurring a performance drop due to misaligned between speech and language representations. To bridge this gap, we propose a joint speech and language model (SLM) using a Speech2Text adapter, which maps speech into text token embedding space without speech information loss. Additionally, using a CTC-based blank-filtering, we can reduce the speech sequence length to that of text. In speech MultiWoz dataset (DSTC11 challenge), SLM largely improves the dialog state tracking (DST) performance (24.7% to 28.4% accuracy). Further to address errors on rare entities, we augment SLM with a Speech2Entity retriever, which uses speech to retrieve relevant entities, and then adds them to the original SLM input as a prefix. With this retrieval-augmented SLM (ReSLM), the DST performance jumps to 34.6% accuracy. Moreover, augmenting the ASR task with the dialog understanding task improves the ASR performance from 9.4% to 8.5% WER.

==> discussion.tex <==
\section{Discussion}

% \texttt{TODO(izhak) 1) High error rate in named entity prediction. 2) Error propagates from ASR transcript to dialog states. 3) Error propagates from the beginning of a dialog to the end.}
% \texttt{(Outperform cascaded model without finetuning with ASR transcript (28.0\% JGA). On par with cascaded model finetuning on ASR transcript (31.8\% JGA). As a byproduct, the retrieval component improve ASR performance. RNN-T ASR model trained on PeopleSpeech corpus: 13\% WER.)
% ReSLM on DST task actually has better WER than on ASR task. }

% Next step:

% \texttt{Large room for improvement in audio retriever; Handle better multi-entities per utterance / long utterances; Better approach to integrate retrieved results Through external memory slot rather than simple prepending, i.e. RETRO, Altas }

% Authors must proofread their PDF file prior to submission, to ensure it is correct. Do not rely on proofreading the \LaTeX\xspace source or Word document. \textbf{Please proofread the PDF file before it is submitted.}
